Sparse Bayesian time-varying covariance estimation in many dimensions

We address the curse of dimensionality in dynamic covariance estimation by modeling the underlying co-volatility dynamics of a time series vector through latent time-varying stochastic factors. The use of a global-local shrinkage prior for the elements of the factor loadings matrix pulls loadings on superfluous factors towards zero. To demonstrate the merits of the proposed framework, the model is applied to simulated data as well as to daily log-returns of 300 S&P 500 members. Our approach yields precise correlation estimates, strong implied minimum variance portfolio performance and superior forecasting accuracy in terms of log predictive scores when compared to typical benchmarks.

==> tables/GMVP_old.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon May 15 13:19:49 2017
\begin{table}[t]
\centering
\begin{tabular}{rrrrr}
  \hline
 & Avg & SD & Sharpe & PLPS \\ 
  \hline
Equal weight portfolio & 0.00 & 29.02 & 0.00 &  \\ 
  MA (500 days) & $-$2.39 & 16.56 & $-$0.14 & $-$966.30 \\ 
 EWMA ($\lambda = 0.94$) & $-$4.43 & 35.90 & $-$0.12 & $-3 \times 10^{9}$ \\ 
  EWMA ($\lambda = 0.99$) & $-$4.18 & 18.42 & $-$0.23 & $-$2056.11 \\ 
  Ledoit-Wolf & 6.14 & 12.53 & 0.49 & $-$620.46 \\ 
  FF+MOM & 12.68 & 16.82 & 0.75 & $-$571.58 \\ 
  SV & 1.02 & 22.53 & 0.05 & $-$646.14 \\ 
  N-FSV 1 & 9.45 & 19.03 & 0.50 & $-$579.85 \\ 
  N-FSV 2 & 9.32 & 18.92 & 0.49 & $-$570.89 \\ 
  N-FSV 3 & 7.36 & 15.50 & 0.48 & $-$564.67 \\ 
  N-FSV 4 & 8.26 & 14.58 & 0.57 & $-$559.07 \\ 
  N-FSV 10 & 12.45 & 12.94 & 0.96 & $-$548.39 \\ 
  N-FSV 20 & 7.81 & 12.57 & 0.62 & $-$544.32 \\ 
  N-FSV 50 & 5.03 & 12.41 & 0.40 & $-$539.57 \\ 
  NG-FSV 1 & 9.44 & 18.98 & 0.50 & $-$579.84 \\ 
  NG-FSV 2 & 9.37 & 18.84 & 0.50 & $-$570.92 \\ 
  NG-FSV 3 & 7.20 & 15.52 & 0.46 & $-$564.75 \\ 
  NG-FSV 4 & 8.36 & 14.85 & 0.56 & $-$559.33 \\ 
  NG-FSV 10 & 12.00 & 12.94 & 0.93 & $-$548.39 \\ 
  NG-FSV 20 & 13.33 & 12.02 & 1.11 & $-$543.84 \\ 
  NG-FSV 50 & 10.78 & 12.42 & 0.87 & $-$538.91 \\ 
   \hline
\end{tabular}
\caption{Predictive performance measures, averaged over $1000$ trading days after 5/3/2006. Avg: Annualized average excess returns over the equal weight portolio. SD: Annualized empirical standard deviations of portfolio returns. Sharpe: Quotients of Avg and SD. PLPS: One-day-ahead pseudo log predictive scores.}
\label{GMVP}
\end{table}

